FENDL: A library for fusion research and applications

The Fusion Evaluated Nuclear Data Library (FENDL) is a comprehensive and validated collection of nuclear cross section data coordinated by the International Atomic Energy Agency (IAEA) Nuclear Data Section (NDS). FENDL assembles the best nuclear data for fusion applications selected from available nuclear data libraries and has been under development for decades. FENDL contains sub-libraries for incident neutron, proton, and deuteron cross sections including general purpose and activation files used for particle transport and nuclide inventory calculations. We describe the history, selection of evaluations for the various sub-libraries (neutron, proton, deuteron) with the focus on transport and reactor dosimetry applications, the processing of the nuclear data for application codes, and the development of the TENDL-2017 library which is the currently recommended activation library for FENDL. We briefly describe the IAEA IRDFF library as the recommended library for dosimetry fusion applications. We also present work on validation of the neutron sub-library using a variety of fusion relevant computational and experimental benchmarks. A variety of cross section libraries are used for the validation work including FENDL-2.1, FENDL-3.1d, FENDL-3.2, ENDF/B-VIII.0, and JEFF-3.2 with the emphasis on the FENDL libraries. The results of the experimental validation showed that the performance of FENDL-3.2b is at least as good and in most cases better than FENDL-2.1. Future work will consider improved evaluations developed by the International Nuclear Data Evaluation Network (INDEN). Additional work will be needed to investigate differences in gas production in structural materials. Covariance matrices need to be updated to support the development of fusion technology. Additional validation work for high-energy neutrons, protons and deuterons, and the activation library will be needed.

==> print-sublib-atom-table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% DO NOT EDIT THIS FILE   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setsublib{atom}


\def\sublibtableheader{
\T\# & Material & Source & Emax & Comment \\
     &          &        & [MeV] &        \\
\hline
}


\begin{table*}
\def\tand{&}
\begin{tabular}{r|llll}
% header
\sublibtableheader
% body
  \ifcounter{it}{}{\newcounter{it}}
  \setcounter{it}{1}
  \whiledo{\theit<62}{
    \theit \tand
	\getmaterial{\theit} \tand
	\getmatattr{\getmaterial{\theit}}{source} \tand
	\getmatattr{\getmaterial{\theit}}{Emax} \tand
	\getmatattr{\getmaterial{\theit}}{comment} \\
    \ifnum\value{it}=61\hline\end{tabular}\fi
  \stepcounter{it}
  }%
 %\par Immediately after the table
  \caption{photoatomic transport sublibrary}
\end{table*}



==> print-sublib-deuteron-table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% DO NOT EDIT THIS FILE   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setsublib{deuteron}

\def\sublibtableheader{
\T\# & Material & Source & Emax & Comment \\
     &          &        & [MeV] &        \\
\hline
}

\begin{table*}
\def\tand{&}
\begin{tabular}{r|llll}
% header
\sublibtableheader
% body
  \ifcounter{it}{}{\newcounter{it}}
  \setcounter{it}{1}
  \whiledo{\theit<50}{
    \theit \tand
	\getmaterial{\theit} \tand
	\getmatattr{\getmaterial{\theit}}{source} \tand
	\getmatattr{\getmaterial{\theit}}{Emax} \tand
	\getmatattr{\getmaterial{\theit}}{comment} \\
    \ifnum\value{it}=49\hline\end{tabular}\fi
  \stepcounter{it}
  }%
 %\par Immediately after the table
  \caption{deuteron transport sublibrary}
\end{table*}


\begin{table*}
\def\tand{&}
\begin{tabular}{r|llll}
% header
\sublibtableheader
% body
  \ifcounter{it}{}{\newcounter{it}}
  \setcounter{it}{50}
  \whiledo{\theit<100}{
    \theit \tand
	\getmaterial{\theit} \tand
	\getmatattr{\getmaterial{\theit}}{source} \tand
	\getmatattr{\getmaterial{\theit}}{Emax} \tand
	\getmatattr{\getmaterial{\theit}}{comment} \\
    \ifnum\value{it}=99\hline\end{tabular}\fi
  \stepcounter{it}
  }%
 %\par Immediately after the table
  \caption{deuteron transport sublibrary}
\end{table*}


\begin{table*}
\def\tand{&}
\begin{tabular}{r|llll}
% header
\sublibtableheader
% body
  \ifcounter{it}{}{\newcounter{it}}
  \setcounter{it}{100}
  \whiledo{\theit<150}{
    \theit \tand
	\getmaterial{\theit} \tand
	\getmatattr{\getmaterial{\theit}}{source} \tand
	\getmatattr{\getmaterial{\theit}}{Emax} \tand
	\getmatattr{\getmaterial{\theit}}{comment} \\
    \ifnum\value{it}=149\hline\end{tabular}\fi
  \stepcounter{it}
  }%
 %\par Immediately after the table
  \caption{deuteron transport sublibrary}
\end{table*}


\begin{table*}
\def\tand{&}
\begin{tabular}{r|llll}
% header
\sublibtableheader
% body
  \ifcounter{it}{}{\newcounter{it}}
  \setcounter{it}{150}
  \whiledo{\theit<176}{
    \theit \tand
	\getmaterial{\theit} \tand
	\getmatattr{\getmaterial{\theit}}{source} \tand
	\getmatattr{\getmaterial{\theit}}{Emax} \tand
	\getmatattr{\getmaterial{\theit}}{comment} \\
    \ifnum\value{it}=175\hline\end{tabular}\fi
  \stepcounter{it}
  }%
 %\par Immediately after the table
  \caption{deuteron transport sublibrary}
\end{table*}


==> section-guidelines.tex <==
This section contains information that is hopefully
pertinent for the drafting of the individual sections.

\subsection{General workflow}
First regarding the general workflow.
The Latex files can be edited online on Overleaf,
even simultaneously by several collaborators.
For people that want to use git to track changes in the document,
and work locally, this is also possible. The command:
\textit{git clone https://git.overleaf.com/6215fb47311847d7ddd5afdf fendl-paper}
downloads all the Latex files, figures and bibliography.
Files can be modified locally and then pushed back. 
If you follow this workflow,
please don't forget to integrate remote changes via \textit{git pull origin}
to your local repository before pushing. 
Furthermore, to avoid problems with simultaneous edits,
each of the sections \textit{Introduction},
\textit{Evaluation}, \textit{Processing}, \textit{Validation},
\textit{Future needs}, and \textit{Conclusions} has been singled out
in a separate Latex file, e.g., \textit{section-evaluation},
\textit{section-validation}, etc. Content associated with these
sections should be added there and NOT in the \textit{main.tex} file.

\subsection{References and citations}
References to a figure, table or equation inside the
paper can be placed using the \textit{\textbackslash{}cref} command,
e.g., \textit{\textbackslash{}cref\{sec:introduction\}} would create
the following reference: \cref{sec:introduction}.
As can be seen, it prefixes the number by the appropriate word,
such as \textit{Section} or \textit{Figure}. This prefix word
can be globally changed if required.

Citations can be inserted by using the \textit{\textbackslash{}cite}
command.The bibliography is stored in the file \textit{main.bib}.
For instance, the report for FENDL-3 which is already stored as
bibliographic item in the bib file can be cited by
\textit{\textbackslash{}cite\{forrestFENDL3LibrarySummary2012\}} and
would produce the following element in the text:
\cite{forrestFENDL3LibrarySummary2012}

\subsection{Figures}
As Nuclear Data Sheets publishes its papers in a two-column format,
the width of figures can either span the width of one column or of
two columns. A figure in one column can have up to 8.69cm, which is
approximately 3.42in. I think we can keep the height more flexible,
but up to 6cm (2.36in) looks reasonable to me. \Cref{fig:one-column-example}
is an example of a one-column figure with width=8.69cm and height=6cm.
\begin{figure}[t!]
\includegraphics[width=8.69cm,height=6cm]{figures/guidelines/blackbox.png}
    \caption{Example of a one column figure with a width of 8.69cm (3.42in)
    and a height of 6cm}
\label{fig:one-column-example}
\end{figure}

Two column figures can also be created by using
\textit{\textbackslash{}begin\{figure*\}} ... \textit{\textbackslash{}and\{figure*\}} environment.
The width of a two-column figure can be 17.75cm (=6.99in). An example
of a two-column figure is given by~\cref{fig:two-column-example}.
\begin{figure*}[b!]
\includegraphics[width=17.75cm,height=5cm]{figures/guidelines/blackbox.png}
\caption{Two-column figure spanning the whole page, here with a width of 17.75cm (6.99in)
and a height of 5cm (1.97in).}
\label{fig:two-column-example}
\end{figure*}

Regarding font sizes in figures, \cref{fig:plot-example} uses 10pt for tick labels and the titles of the axes.
As plot programs are different, it may be difficult to agree on a precise size but if we manage
to have similar font sizes for the plots, that should be good enough.
\begin{figure}
    \includegraphics{figures/guidelines/example_plot.png}
    \caption{Some example plot with the size of tick and axis labels being 10pt}
    \label{fig:plot-example}
\end{figure}

\subsection{Tables}

Here is an example of a table spanning one column.

\begin{table}[!hbtp]
\vspace{-2mm}
\caption{Reaction Q-values and thresholds} \label{Q-values}
\begin{tabular}{r | l l | c r r} \hline \hline
\T \#&    Reaction                   & Reaction& MAT   & Q-Value & Eff. Thr.    \\
    &                                & ~~~ID   &       & [keV]   & [keV]        \\ \hline
\T 1& $^{10}$B(n,$\alpha$)$^{7}$Li   & B10a    & 525   & 2789.323&  0.0         \\
2   & $^{47}$Ti(n,p)$^{47}$Sc        & Ti47p   & 2228  & 181.580 &  800.0       \\
3   & $^{54}$Fe(n,p)$^{54}$Mn        & Fe54p   & 2625  & 85.2127 &  0.0         \\
4   & $^{54}$Fe(n,$\alpha$)$^{51}$Cr & Fe54a   & 2625  & 842.760 &  0.0         \\
5   & $^{58}$Ni(n,p)$^{58}$Co        & Ni58p   & 2825  & 400.800 &  400.0       \\
6   & $^{59}$Co(n,$\alpha$)$^{56}$Mn & Co59a   & 2725  & 328.400 &  334.016     \\
7   & $^{63}$Cu(n,$\alpha$)$^{60}$Co & Cu63a   & 2925  & 1714.400&  2250.0      \\
8   & $^{64}$Zn(n,p)$^{64}$Cu        & Zn64p   & 3025  & 203.500 &  500.0       \\
9   & $^{67}$Zn(n,p)$^{67}$Cu        & Zn67p   & 3034  & 220.690 &  0.0         \\
10  & $^{92}$Mo(n,p)$^{92m}$Nb       & MoNb92pm& 4225  & 425.680 &  1000.0      \\ \hline \hline
\end{tabular}
\vspace{-6mm}
\end{table}



==> sublib-table-macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% DO NOT EDIT THIS FILE   %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatletter

% set the sublibrary for which the materials are registered
\newcommand{\setsublib}[1]{
  \def\cursublib{#1}
  \def\curcountername{matcnt+\cursublib}
  \ifcounter{\curcountername}{}{\newcounter{\curcountername}}
}

\newcommand{\stepsublibcnt}{
  \stepcounter{\curcountername}
}

\newcommand{\getsublibcnt}{%
  \arabic{\curcountername}%
}

% register a material to be plotted in the table
\newcommand{\registermaterial}[1]{%
  \stepcounter{\curcountername}%
  \@namedef{matlist+\cursublib+\getsublibcnt}{#1}%
}

% get element at specific position in list
\newcommand\getmaterial[1]{%
  \@nameuse{matlist+\cursublib+#1}%
}

% convenience function for retrieving an attribute of a material 
\newcommand\getmatattr[2]{%
  \ifcsname \cursublib+#1+#2\endcsname%
    \csname \cursublib+#1+#2\endcsname%
  \else%
    %{\color{red}Missing}%
  \fi%
}

\newcommand\setmatattr[3]{
    \expandafter\def\csname \cursublib+#1+#2\endcsname{#3}
}

% helpful to check if a counter exists
\newcommand*\ifcounter[1]{%
  \ifcsname c@#1\endcsname
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\makeatother

==> validationtext/experimentalbenchmarks/subsectionRezMoved2Schulc.tex <==
\subsubsection{Validation in Research Center Rez}

Michal Košťál and Martin Schulc

\begin{enumerate}
\def\labelenumi{\alph{enumi})}
\item
  \textbf{Validation of dosimetric libraries}
\end{enumerate}

The dosimetric cross sections are fundamental quantities for proper
determination of the neutron fluxes. They are essential in the correct
determination of neutron fluxes. In fusion applications it is important
to validate this quantity especially in regions close to a fusion
neutron energy spectrum. Activation reactions which are dosimetric are
taken from IRDFF-II as it is the recommended dosimetry library for
reaction dosimetry and fusion. The presented set of validations was
realized in neutron quasi monoenergetic neutron field formed by proton
irradiation of thin Li target with protons of energies 12.4 and 14.4
MeV. The neutron spectra are shown in Figure 1. The neutron spectrum was
measured in position approximately 4 m from neutron source formed by
\textsuperscript{nat.}Li target irradiated by protons. The activation
experiment was realized simultaneously with measurement of neutron
spectrum. To achieve a sufficient activation, the experiment was
realized in close distance to target assembly. Due to relatively large
volume of materials in vicinity of target assembly, the neutron spectrum
in the irradiated foils differs from spectrum measured far from target.
The correction factor, in form of ratios between spectrum in measuring
position and spectrum in the target was determined by simulation, and
these ratios were used to transform the measured neutron spectra from
the position of scintillator detectors to the position of activation
foils (8.6 cm from Li target). The flux was normalized using Al and Ni
monitors using \textsuperscript{27}Al(n,) and
\textsuperscript{58}Ni(n,p) reactions. These evaluated neutron fluxes in
the target are useable for determination of evaluated reaction rates by
folding of this evaluated spectrum with selected nuclear data library.
The details of methodology can be found in
\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bib27}{Matej
et al., 2022}.

{{[}CHART{]}}

Figure 1.: Neutron spectra in both tested cases, neutrons induced by
14.4 and 12.4 MeV protons interacting with \textsuperscript{nat.}Li
target

Using the time evolution of activation and final activity obtained in
the irradiation experiment, the reaction rates were derived. This
experimentally obtained reaction rates were compared with evaluated
reaction rates obtained by folding of the evaluated neutron spectra in
target with selected nuclear data library. This methodology was used for
testing of large set of commonly used dosimetry reactions. There were
tested data from IRDFF-II ({Trkov et al., 2020}), ENDF/B-VIII ({Brown et
al., 2018}), JEFF-3.3 ({Koning, et al., 2010}) and JENDL-4 ({Shibata et
al. 2011}) data libraries. In common dosimetry reactions, clearly the
best agreement was reached using the IRDFF-II evaluation. All used
IRDFF-II reactions are within two sigma uncertainty and other tested
libraries have several reactions with higher discrepancy. The most
discrepant is \textsuperscript{19}F(n,2n) in JENDL-4, where the
discrepancy is higher than ten sigma.

Table 1: Validation of selected reaction rates in
\textsuperscript{7}Li(p,n) field from 12.4 MeV protons by means of C/E-1
comparison
(\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bib27}{Matej
et al., 2022})

\begin{longtable}[]{@{}lllllll@{}}
\toprule
Reaction & E\textsubscript{50\%} {[}MeV{]} & IRDFF-II & JEFF-3.3 &
JENDL-4 & ENDF/B-VIII.0 & Unc.\tabularnewline
\midrule
\endhead
\textsuperscript{54}Fe(n,p) & 6.78 & 1.9 \% & -2.3 \% & 5.2 \% & 2.0 \%
& 4.2 \%\tabularnewline
\textsuperscript{47}Ti(n,p) & 7.43 & 7.8 \% & 8.4 \% & 11.7 \% & 23.6 \%
& 3.7 \%\tabularnewline
\textsuperscript{46}Ti(n,p) & 9.61 & 11.7 \% & 12.2 \% & 9.8 \% & 4.8 \%
& 8.3 \%\tabularnewline
\textsuperscript{59}Co(n,p) & 10.05 & 3.2 \% & -7.1 \% & -5.5 \% & 3.2
\% & 4.1 \%\tabularnewline
\textsuperscript{60}Ni(n,p) & 10.25 & 18.1 \% & 18.8 \% & 20.9 \% & 18.1
\% & 6.9 \%\tabularnewline
\textsuperscript{56}Fe(n,p) & 10.30 & -2.5 \% & -4.0 \% & 0.2 \% & -2.5
\% & 3.9 \%\tabularnewline
\textsuperscript{24}Mg(n,p) & 10.37 & 3.7 \% & 8.4 \% & 10.3 \% & 7.7 \%
& 4.1 \%\tabularnewline
\textsuperscript{59}Co(n,α) & 10.43 & -1.9 \% & -4.6 \% & 1.0 \% & 1.7
\% & 4.0 \%\tabularnewline
\textsuperscript{48}Ti(n,p) & 10.45 & -0.5 \% & 0.1 \% & -1.9 \% & 10.6
\% & 4.1 \%\tabularnewline
\textsuperscript{51}V(n,α) & 10.57 & -1.7 \% & -1.2 \% & 8.4 \% & 12.2
\% & 5.3 \%\tabularnewline
\textsuperscript{197}Au(n,2n) & 10.60 & -3.4 \% & -5.5 \% & 22.6 \% &
-6.1 \% & 4.3 \%\tabularnewline
\textsuperscript{58}Ni(n,x)\textsuperscript{57}Co & 10.89 & - & -20.9 \%
& -10.6 \% & -18.1 \% & 3.7 \%\tabularnewline
\textsuperscript{59}Co(n,2n) & 11.27 & -2.7 \% & -2.7 \% & 11.7 \% &
14.0 \% & 6.2 \%\tabularnewline
\bottomrule
\end{longtable}

Table 2: Validation of selected reaction rates in 7Li(p,n) field from
14.4 MeV protons by means of C/E-1 comparison
(\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bib27}{Matej
et al., 2022})

\begin{longtable}[]{@{}lllllll@{}}
\toprule
Reaction & E\textsubscript{50\%} {[}MeV{]} & IRDFF-II & JEFF-3.3 &
JENDL-4 & ENDF/B-VIII.0 & Unc.\tabularnewline
\midrule
\endhead
\textsuperscript{54}Fe(n,p) & 7.75 & -1.2 \% & -3.0 \% & 0.6 \% & -1.0
\% & 3.9 \%\tabularnewline
\textsuperscript{47}Ti(n,p) & 8.37 & 1.3 \% & 1.3 \% & 2.1 \% & 15.9 \%
& 6.8 \%\tabularnewline
\textsuperscript{46}Ti(n,p) & 10.04 & 7.8 \% & 7.8 \% & 2.9 \% & 4.2 \%
& 4.1 \%\tabularnewline
\textsuperscript{59}Co(n,p) & 12.13 & 7.2 \% & -1.7 \% & -1.3 \% & 4.8
\% & 4.6 \%\tabularnewline
\textsuperscript{60}Ni(n,p) & 12.24 & 3.8 \% & 1.2 \% & 7.9 \% & 9.8 \%
& 5.3 \%\tabularnewline
\textsuperscript{54}Fe(n,α) & 12.29 & -5.4 \% & -17.4 \% & -5.5 \% &
-61.7 \% & 6.4 \%\tabularnewline
\textsuperscript{24}Mg(n,p) & 12.31 & 3.0 \% & 10.1 \% & 10.1 \% & 10.1
\% & 5.0 \%\tabularnewline
\textsuperscript{56}Fe(n,p) & 12.31 & -1.7 \% & -2.5 \% & -3.9 \% & -1.6
\% & 5.0 \%\tabularnewline
\textsuperscript{59}Co(n,α) & 12.40 & -2.9 \% & -5.0 \% & -3.2 \% & -0.9
\% & 5.3 \%\tabularnewline
\textsuperscript{48}Ti(n,p) & 12.41 & 2.2 \% & 2.3 \% & -3.9 \% & 0.5 \%
& 5.4 \%\tabularnewline
\textsuperscript{51}V(n,α) & 12.50 & -4.8 \% & -5.0 \% & -0.4 \% & 1.5
\% & 6.3 \%\tabularnewline
\textsuperscript{197}Au(n,2n) & 12.50 & 2.9 \% & 4.2 \% & 16.0 \% & 4.2
\% & 6.2 \%\tabularnewline
\textsuperscript{58}Ni(n,x)\textsuperscript{57}Co & 12.57 & - & -7.7 \%
& 2.5 \% & -10.2 \% & 6.6 \%\tabularnewline
\textsuperscript{59}Co(n,2n) & 12.58 & -7.2 \% & -6.4 \% & -13.5 \% &
-4.0 \% & 6.7 \%\tabularnewline
\textsuperscript{19}F(n,2n) & 12.64 & 10.7 \% & 40.1 \% & 75.7 \% & 40.1
\% & 7.3 \%\tabularnewline
\textsuperscript{55}Mn(n,2n) & 12.58 & -2.8 \% & 4.9 \% & -1.0 \% & -3.9
\% & 6.8 \%\tabularnewline
\bottomrule
\end{longtable}

\begin{enumerate}
\def\labelenumi{\alph{enumi})}
\setcounter{enumi}{1}
\item
  \textbf{Validation of transport FENDL libraries}
\end{enumerate}

The neutron transport in various important materials was tested using
\textsuperscript{252}Cf(s.f) neutron source. The
\textsuperscript{252}Cf(s.f) is a neutron standard (Trkov et al 2020),
thus there are low uncertainties in its spectrum, thus discrepancies in
neutron spectra after passing by material layer can be accounted to
discrepancies in cross section description of the studied material. The
method of \textsuperscript{252}Cf(s.f) in our institute was profoundly
summarized in (Schulc et al., 2019). The materials tested were Copper,
Nickel, Iron, lead and Stainless steel. The nickel and iron were in form
of sphere of diameter 50cm, the copper and stainless steel in form of
block. The copper block had dimensions of 48 x 49.5 x 49.5 cm, while the
stainless steel block dimensions were 50.4 x 50.2 x 50.2 cm. The lead
block had dimensions of 52.5 x 52.5 x 10 cm. Nickel and iron validation was
performed in the spheres of 50 cm diameter. The validation process was
divided into two parts, measurement of the neutron spectra in the region
of 1-12 MeV and measurement of the reaction rates of the activated
materials. Reactions were carefully selected, i.e. only IRDFF-II
validated dosimetric reactions were used for the validation of FENDL
transport libraries. All calculations were performed using MCNP6.2
transport code ({Goorley et al., 2012)}.

\textbf{Neutron spectra measurement by proton recoil method}

The leakage neutron fluxes were monitored using stilbene scintillation
detector of diameter 1 cm and length of 1 cm. The spectra were measured
in the distance of 100 cm from the centre of the neutron source. The
used spectrometric system
(\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bib28}{Matěj,
2014},~\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bib37}{Veškrna
et al., 2014}) features two-parameter data processing from scintillation
detectors in mixed gamma and neutron fields. In addition to the basic
data acquisition and parameter settings for individual experiments, the
control software contains mathematical evaluation algorithms that select
the relevant data from the multi-parameter raw data
(\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bib10}{Cvachovec
and Cvachovec, 2008}). Using this method it is possible to evaluate
individual components separately, i.e. neutrons and gammas. More details
concerning separation properties can be found
in~\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bib27}{Matej
et al., 2021}. The plot of the pulse shape discrimination is shown in
Figure 2 below. The neutron and gamma signals are well separated because
even in region below 1 MeV the overlaping of neutron and gamma pulses is
has low frequency, see Figure 3.

\includegraphics[width=4.27083in,height=4.01003in]{media/image1.png}

Figure 2.: Neutron gamma discrimination in stainless steel cube
measurement

\includegraphics[width=6.11458in,height=2.66502in]{media/image2.png}

Figure 3.: Discrimination between gammas (right) and neutrons (left) in
30 channel \textasciitilde{} 0.8 MeV.

Leakage validation by means of reaction rates measurement

The leakage flux was monitored also by means of reaction rates. The
reaction rates were derived from Net Peak Areas (NPA) from radioisotopes
induced in activation foils attached to the block surface or put inside
the blocks. The NPAs were measured with well described HPGe efficiency
and energetic calibration. The good description allows computational
determination of efficiency. There were used relatively big foils and
the measurement was realized in HPGE end cap position. More details
concerning gamma spectrometry can be found in (Kostal et al 2017).

Neutron leakage from copper block:

The copper block has dimensions: 48 cm length, 49.5 cm width, and 49.5
cm height. The neutron spectrum is measured in the distance of 100 cm
from the centre of the source in source plane. In the case of copper neutron leakage,
higher flux is predicted can be observed in energy region under 5 MeV.
In higher regions the agreement in FENDL-2.1 and 3.2 are even better
than in ENDF/B-VIII.0 case, see Figure 4. More details can be found in
Schulc et al., 2022a.

{{[}CHART{]}}

Figure 4.: Neutron leakage spectra comparison for different libraries.

The activation foils were attached to the thin aluminium foil, and
placed into the copper block at the distance of 16 cm from the
\textsuperscript{252}Cf neutron source centre. The experiment
specifically focuses on
\textsuperscript{58}Ni(n,p)\textsuperscript{58}Co,
\textsuperscript{93}Nb(n,2n)\textsuperscript{92m}Nb,
\textsuperscript{197}Au(n,g)\textsuperscript{198}Au and
\textsuperscript{55}Mn(n,g)\textsuperscript{56}Mn dosimetry reactions.
Table 3 summarizes obtained results. Results are similar as for
ENDF/B-VIII.0 library. More details concerning the experiment can be
found in Schulc et al., 2021.

Table 3: Copper benchmark activation foils.

\begin{longtable}[]{@{}lllll@{}}
\toprule
Reaction & ENDF/B-VIII.0 & FENDL-3.2 & FENDL-2.1 & Experimental
uncertainty\tabularnewline
\midrule
\endhead
197Au(n,g) I & -16.1\% & -14.3\% & -14.6\% & 3.8\%\tabularnewline
197Au(n,g) II & -7.8\% & -6.1\% & -6.1\% & 3.9\%\tabularnewline
63Cu(n,g) I & -33.8\% & -40.1\% & -39.8\% & 4.2\%\tabularnewline
63Cu(n,g) II & -55.6\% & -60.4\% & -60.3\% & 4.1\%\tabularnewline
55Mn(n,g) & -4.8\% & -2.3\% & -0.8\% & 4.5\%\tabularnewline
93Nb(n,2n) & -13.69\% & -1.86\% & -1.86\% & 4.7\%\tabularnewline
58Ni(n,p) & 5.22\% & 28.1\% & 28.1\% & 4.1\%\tabularnewline
\bottomrule
\end{longtable}

Neutron leakage from nickel sphere, diameter of 50 cm

The fast leakage neutron spectra have been measured on spherical nickel
benchmark assembly of diameter 50 cm. The \textsuperscript{252}Cf
neutron source with was placed into the centre of the sphere. FENDL-3.2b
agrees with experimental results very well in the region above 3 MeV,
see Figure 5. Performance below 3 MeV is much worse. Table 4 summarizes
C/E-1 for all activation foils on the nickel sphere surface.

Table 4: Results for activation foils on the nickel sphere surface

\begin{longtable}[]{@{}lllll@{}}
\toprule
Reaction & ENDF/B-VIII.0 & FENDL-2.1 & FENDL-3.2b &
Uncertainty\tabularnewline
\midrule
\endhead
115In(n,n') & -21.0\% & 2.9\% & -5.8\% & 4.2\%\tabularnewline
115In(n,g) & 10.0\% & 19.8\% & 26.3\% & 4.4\%\tabularnewline
58Ni(n,p) & -0.6\% & 13.7\% & 19.3\% & 5.0\%\tabularnewline
55Mn(n,g) & -26.1\% & 8.3\% & 13.4\% & 5.5\%\tabularnewline
\bottomrule
\end{longtable}

{{[}CHART{]}}

Figure 5.: Neutron leakage spectra comparison for different libraries.

Neutron leakage from iron sphere, diameter of 50 cm

The fast leakage neutron spectra have been measured on spherical nickel
benchmark assembly of diameter 50 cm. The \textsuperscript{252}Cf
neutron source with was placed into the centre of the sphere. Table 5
shows obtained results for activation foils on the iron sphere surface.
FENDL-3.2b gives better results than FENDL-2.1. Overall agreement is not
achieved with any library. Figure 6 compares neutron leakage fluxes in
different libraries. FENDL-3.2b library agrees better with experiment
than FENDL-2.1. Reasonable agreement is achieved above 4 MeV.

Table 5: Results for activation foils on the iron sphere surface.

\begin{longtable}[]{@{}llllll@{}}
\toprule
& ENDF/B-VIII.0 & JEFF-3.3 & FENDL-3.2b & FENDL-2.1 &
Unc.\tabularnewline
\midrule
\endhead
115In(n,n') & -18.1\% & -2.2\% & 1.7\% & 13.9\% & 4\%\tabularnewline
115In(n,g) & 62.8\% & 29.9\% & 50.2\% & 24.9\% & 5\%\tabularnewline
58Ni(n,p) & -11.9\% & 15.0\% & 16.3\% & 48.3\% & 6\%\tabularnewline
55Mn(n,g) & -28.3\% & -43.7\% & -26.3\% & -41.9\% & 6\%\tabularnewline
\bottomrule
\end{longtable}

{{[}CHART{]}}

Figure 6: Neutron leakage spectra comparison for different libraries.

Neutron leakage from stainless steel block

The validation was performed by means of samples activation in different
positions and also the measurement of the fast neutron spectrum in the
energy range of 1-12 MeV using a scintillation stilbene detector.
Stainless steel was used in the form of a block with a hole for the
neutron source. Table 6 summarizes C/E-1 for activation foil on the
stainless steel block surface. Figure 7 compares neutron leakage fluxes
in different libraries. FENDL-3.2b library agrees well with experiment
above 4 MeV. ENDF/B-VIII.0 performs much worse in this region.

Table 6 : Stainless steel

\begin{longtable}[]{@{}lll@{}}
\toprule
Reaction & Front side & Lateral side\tabularnewline
\midrule
\endhead
ENDF/B-VIII.0 & -18.40\% & -18.50\%\tabularnewline
JEFF-3.3 & 2.30\% & 5.50\%\tabularnewline
JENDL-4 & -5.40\% & -3.40\%\tabularnewline
FENDL-2.1 & -0.70\% & -0.70\%\tabularnewline
FENDL-3.2 & -3.80\% & -4.90\%\tabularnewline
Unc. & 4.57\% & 3.24\%\tabularnewline
\bottomrule
\end{longtable}

{{[}CHART{]}}

Figure 7.: Neutron leakage spectra comparison for different libraries.

Neutron leakage from lead block

In the irradiation setup,the samples were placed behind 5 and 10 cm of
the lead material. Samples were measured using a gamma spectrometry to
infer the reaction rate and compared with MCNP6 calculations using
ENDF/B-VIII.0 lead cross sections. The experiment used validated
IRDFF-II dosimetric reactions to validate lead cross sections, namely
\textsuperscript{197}Au(n,2n)\textsuperscript{196}Au,
\textsuperscript{58}Ni(n,p)\textsuperscript{58}Co,
\textsuperscript{93}Nb(n,2n)\textsuperscript{92m}Nb,
\textsuperscript{115}In(n,n´)\textsuperscript{115m}In,
\textsuperscript{115}In(n,γ)\textsuperscript{116m}In,
\textsuperscript{197}Au(n,γ)\textsuperscript{198}Au and
\textsuperscript{63}Cu(n,γ)\textsuperscript{64}Cu reactions. The
threshold reactions agree reasonably with calculations; however, the
experimental data suggests a higher thermal neutron flux behind lead
bricks. Table 7 summarizes C/E-1 for all activation foils. More details
can be found in Schulc et al., 2022b.

Table 7: Calculation and C/E-1 comparison for all reactions inside lead
bricks.

\begin{longtable}[]{@{}llllll@{}}
\toprule
\endhead
Reaction & Lead thickness & C/E-1 (FENDL-2.1) & C/E-1 (FENDL-3.2) &
C/E-1 (ENDF/B-VIII.0) & Exp. Uncertainty\tabularnewline
\textsuperscript{58}Ni(n,p)\textsuperscript{58}Co & 10 cm & -2.16\% &
+1.71\% & +6.6\% & 3.2\%\tabularnewline
\textsuperscript{93}Nb(n,2n)\textsuperscript{92m}Nb & 10 cm & +6.09\% &
+0.49\% & +2.9\% & 4.2\%\tabularnewline
\textsuperscript{197}Au(n,γ)\textsuperscript{198}Au & 5 cm & -13.9\% &
-15.2\% & -15.8\% & 2.9\%\tabularnewline
\textsuperscript{197}Au(n,γ)\textsuperscript{198}Au & 10 cm & -51.61\% &
-51.8\% & -51.4\% & 3.1\%\tabularnewline
\textsuperscript{197}Au(n,2n)\textsuperscript{196}Au & 5 cm & -0.45\% &
+4.94\% & -0.5\% & 4.1\%\tabularnewline
\textsuperscript{197}Au(n,2n)\textsuperscript{196}Au & 10 cm & +5.54\% &
-1.45\% & +2.4\% & 4.3\%\tabularnewline
\textsuperscript{63}Cu(n,γ)\textsuperscript{64}Cu & 5 cm & +0.76\% &
-1.91\% & -1.1\% & 3.7\%\tabularnewline
\textsuperscript{115}In(n,n´)\textsuperscript{115m}In & 10 cm & -3.95\%
& -1.81\% & +0.2\% & 3.4\%\tabularnewline
\textsuperscript{115}In(n,γ)\textsuperscript{116m}In & 10 cm & -38.23\%
& -38.07\% & -37.9\% & 3.1\%\tabularnewline
\bottomrule
\end{longtable}

References:

{Brown et al., 2018,} D.A. Brown, M.B. Chadwick, R. Capote et al,
"ENDF/B-VIII.0.0: The 8th Major Release of the Nuclear Reaction Data
Library with CIELO-project Cross Sections, New Standards and Thermal
Scattering Data",
\href{http://dx.doi.org/10.1016/j.nds.2011.11.002\#_blank}{Nucl. Data
Sheets, 148 (2018), pp. 1--142.}

{Chadwick et al. 2011,} M.B. Chadwick, M. Herman, P. Obložinský et al,
"ENDF/B-VII.1: Nuclear Data for Science and Technology: Cross Sections,
Covariances, Fission Product Yields and Decay Data",
\href{http://dx.doi.org/10.1016/j.nds.2011.11.002\#_blank}{Nucl. Data
Sheets, 112, (2011), pp. 2887--2996.}

{\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bbib10}{Cvachovec
and Cvachovec, 2008},} J.~Cvachovec,~F.~Cvachovec, Maximum likelihood
estimation of a neutron spectrum and associated uncertainties, Adv. Mil.
Technol.,~3~(2008), pp.~67-79

{Goorley et al., 2012}, T. Goorley et al. "Initial MCNP6 Release
Overview", Nucl. Techn.~180 (2012) pp. 298-315.

{Koning, et al., 2010}, A. J. Koning, et al. "Status of the JEFF Nuclear
Data Library", Proceedings of the International Conference on Nuclear
Data for Science and Technology, Jeju Island, Korea, 2010, p.1057

{Košťál et al., 2017,} M. Košťál, M. Schulc { } et al., Validation of
zirconium isotopes (n,g) and (n,2n) cross sections in a comprehensive
LR-0 reactor operative parameters set, Applied Radiation and Isotopes
128, pp. 92-100, (2017).

{Mannhart 2008,} W. Mannhart, ``Status of the Evaluation of the Neutron
Spectrum of \textsuperscript{252}Cf(sf)'', IAEA Technical Report
INDC(NDS)-0540, IAEA, Vienna (2008). Presentation available at
www-nds.iaea.org/standards-cm-oct-2008/6.PDF

{\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bbib28}{Matěj
2022},} Z.~Matěj et al., The methodology for validation of cross
sections in quasi monoenergetic neutron field, will be published in
NIM-A

{\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bbib28}{Matěj
2014},} Z.~Matěj, Digitalization of Spectrometric System for Mixed Field
of Radiation, LAP LAMBERT Academic Publishing~(2014).

{\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bbib27}{Matej
et al., 2021},} Z.~Matej, F.~Mravec, A.~Jančar, M.~Kostal, F.~Kucera,
F.~Cvachovec, V.~Prenosil, Z.~Kopecky, J.~Culen, O.~Pecak\textbf{,}
Comparison of neutron-Gamma separation qualities of various organic
scintillation materials and liquid scintillator LSB-200\textbf{,} J.
Nucl. Eng. Radiat. Sci.,~7~(2)~(2021), p.~24502

{Pl}{ompen et al., (2020)} A. J. M. Plompen, O. Cabellos, C. De Saint
Jean, M. Fleming, A. Algora, M. Angelone et al., The joint evaluated
fission and fusion nuclear data library, JEFF-3.3. The European Physical
Journal A, 56(7) (2020).

{Schulc et al., 2019}, M. Schulc, M. Kostal et al., "Application of
\textsuperscript{252}Cf neutron source for precise nuclear data
experiments", Applied Radiation and Isotopes, 151, (2019), pp. 187-195.

\hypertarget{schulc-et-al.-2021-m.-schulc-m.-kostal-et-al.-copper-neutron-transport-libraries-validation-by-means-of-a-252cf-standard-neutron-source-nuclear-engineering-and-technology-volume-53-issue-10-october-2021-pages-3151-3157}{%
\subsection{\texorpdfstring{{Schulc et al., 2021}, M. Schulc, M. Kostal
et al., Copper neutron transport libraries validation by means of
a~252Cf standard neutron source,
\href{https://www.sciencedirect.com/journal/nuclear-engineering-and-technology}{Nuclear
Engineering and Technology},
\href{https://www.sciencedirect.com/journal/nuclear-engineering-and-technology/vol/53/issue/10}{Volume
53, Issue 10},~October 2021, Pages
3151-3157}{Schulc et al., 2021, M. Schulc, M. Kostal et al., Copper neutron transport libraries validation by means of a~252Cf standard neutron source, Nuclear Engineering and Technology, Volume 53, Issue 10,~October 2021, Pages 3151-3157}}\label{schulc-et-al.-2021-m.-schulc-m.-kostal-et-al.-copper-neutron-transport-libraries-validation-by-means-of-a-252cf-standard-neutron-source-nuclear-engineering-and-technology-volume-53-issue-10-october-2021-pages-3151-3157}}

{Shibata et al. 2011} K. Shibata, O. Iwamoto, T. Nakagawa, N. Iwamoto,
A. Ichihara, S. Kunieda, S. Chiba, K. Furutaka, N. Otuka, T. Ohsawa, T.
Murata, H. Matsunobu, A. Zukeran, S. Kamada, J. Katakura, JENDL-4.0: A
new library for nuclear science and engineering, J. Nucl. Sci. Technol.,
48 (2011), pp. 1--30

\hypertarget{schulc-et-al.-2022a-m.-schulc-m.-kostal-et-al.-fast-neutron-spectra-measurement-in-a-copper-using-a-252cf-standard-neutron-source-radiation-physics-and-chemistry-volume-192-march-2022-109871}{%
\subsection{\texorpdfstring{{Schulc et al., 2022a,} M. Schulc, M. Kostal
et al., Fast neutron spectra measurement in a copper using a~252Cf
standard neutron source,
\href{https://www.sciencedirect.com/journal/radiation-physics-and-chemistry}{Radiation
Physics and Chemistry},
\href{https://www.sciencedirect.com/journal/radiation-physics-and-chemistry/vol/192/suppl/C}{Volume
192},~March 2022,
109871}{Schulc et al., 2022a, M. Schulc, M. Kostal et al., Fast neutron spectra measurement in a copper using a~252Cf standard neutron source, Radiation Physics and Chemistry, Volume 192,~March 2022, 109871}}\label{schulc-et-al.-2022a-m.-schulc-m.-kostal-et-al.-fast-neutron-spectra-measurement-in-a-copper-using-a-252cf-standard-neutron-source-radiation-physics-and-chemistry-volume-192-march-2022-109871}}

\hypertarget{schulc-et-al.-2022b-m.-schulc-m.-kostal-et-al.-validation-of-the-neutron-lead-transport-for-fusion-applications-volume-54-issue-3-march-2022-pages-959-964.}{%
\section{\texorpdfstring{{Schulc et al., 2022b,} M. Schulc, M. Kostal et
al., Validation of the neutron lead transport for fusion applications,
\href{https://www.sciencedirect.com/journal/nuclear-engineering-and-technology/vol/54/issue/3}{Volume
54, Issue 3},~March 2022, Pages
959-964.}{Schulc et al., 2022b, M. Schulc, M. Kostal et al., Validation of the neutron lead transport for fusion applications, Volume 54, Issue 3,~March 2022, Pages 959-964.}}\label{schulc-et-al.-2022b-m.-schulc-m.-kostal-et-al.-validation-of-the-neutron-lead-transport-for-fusion-applications-volume-54-issue-3-march-2022-pages-959-964.}}

{Trkov et al., 2020,} A. Trkov, P.J. Griffin, S.P. Simakov, L.R.
Greenwood, K.I. Zolotarev, R. Capote et al., ``IRDFF-II: An Updated
Neutron Metrology Library,'' Nuclear Data Sheets 163, 1-108, (2020).

\href{https://www.sciencedirect.com/science/article/pii/S0969806X21001250\#bbib37}{{Veškrna
et al., 2014}}
M.~Veškrna,~Z.~Matěj,~F.~Mravec,~V.~Přenosil,~F.~Cvachovec,~M.~Košťál,
Digitalized two parametric system for gamma/neutron spectrometry RPSD
2014: 18th Topical Meeting of the Radiation Protection \& Shielding
Division of ANS,~American Nuclear Society, Inc,~La Grange Park,
Illinois~(2014), pp.~14-18


